LLM-Assisted Rule Based Machine Translation for Low/No-Resource Languages

We propose a new paradigm for machine translation that is particularly useful for no-resource languages (those without any publicly available bilingual or monolingual corpora): LLM-RBMT (LLM-Assisted Rule Based Machine Translation). Using the LLM-RBMT paradigm, we design the first language education/revitalization-oriented machine translator for Owens Valley Paiute (OVP), a critically endangered Indigenous American language for which there is virtually no publicly available data. We present a detailed evaluation of the translator's components: a rule-based sentence builder, an OVP to English translator, and an English to OVP translator. We also discuss the potential of the paradigm, its limitations, and the many avenues for future research that it opens up.

==> tab_conj.tex <==
\begin{table*}[h!]
    \begin{minipage}{.6\linewidth}
        \centering
        \begin{tabular}{|lr|c|c|c|}
            \hline
            & \textbf{Pronoun} & \textbf{-er Verb} & \textbf{-ir Verb} & \textbf{-ar Verb} \\
            \hline
             &        & com\textbf{er}       & viv\textbf{ir}        & habl\textbf{ar}     \\
            I & Yo       & com\textbf{o}       & viv\textbf{o}        & habl\textbf{o}     \\
            You & Tú       & com\textbf{es}      & viv\textbf{es}       & habl\textbf{as}    \\
            He/She & Él/Ella  & com\textbf{e}       & viv\textbf{e}        & habl\textbf{a}     \\
            We & Nosotros & com\textbf{emos} & viv\textbf{imos}   & habl\textbf{amos}  \\
            You (pl.) & Vosotros & com\textbf{éis}  & viv\textbf{ís}    & habl\textbf{áis}   \\
            They & Ellos/Ellas    & com\textbf{en}    & viv\textbf{en}     & habl\textbf{an}    \\
            \hline
        \end{tabular}
        \caption{Present-tense conjugations for verbs in Spanish}\label{tab:conj}
    \end{minipage}
    \begin{minipage}{.4\linewidth}
        \centering
        \begin{tabular}{|c|c|}
            \hline
            \textbf{Spanish} & \textbf{English} \\
            \hline
            comer & to eat \\
            beber & to drink \\
            hablar & to speak \\
            comprar & to buy \\
            usar & to use \\
            vivir & to live \\
            abrir & to open \\
            \hline
        \end{tabular}
        \caption{List of verbs}\label{tab:verbs}
    \end{minipage}
\end{table*}
